Peer-inspired Student Performance Prediction in Interactive Online Question Pools with Graph Neural Network

Student performance prediction is critical to online education. It can benefit many downstream tasks on online learning platforms, such as estimating dropout rates, facilitating strategic intervention, and enabling adaptive online learning. Interactive online question pools provide students with interesting interactive questions to practice their knowledge in online education. However, little research has been done on student performance prediction in interactive online question pools. Existing work on student performance prediction targets at online learning platforms with predefined course curriculum and accurate knowledge labels like MOOC platforms, but they are not able to fully model knowledge evolution of students in interactive online question pools. In this paper, we propose a novel approach using Graph Neural Networks (GNNs) to achieve better student performance prediction in interactive online question pools. Specifically, we model the relationship between students and questions using student interactions to construct the student-interaction-question network and further present a new GNN model, called R^2GCN, which intrinsically works for the heterogeneous networks, to achieve generalizable student performance prediction in interactive online question pools. We evaluate the effectiveness of our approach on a real-world dataset consisting of 104,113 mouse trajectories generated in the problem-solving process of over 4000 students on 1631 questions. The experiment results show that our approach can achieve a much higher accuracy of student performance prediction than both traditional machine learning approaches and GNN models.

==> src/evaluation.tex <==
\section{Evaluation Metrics} \label{evaluation}
In our experiments, we apply 3 evaluation metrics to compare the performance of different models. We will explain them in detail in this section. Here we use $s$, $n_{c}^s$, $n^s$, $W\mhyphen F1^{s}$ to denote a student, number of the student's correctly predicted questions, number of the student's questions in his test set and the weighted F1 of that student's prediction results. There are totally $N$ students in the dataset.
\paragraph{Average personal accuracy}
Average personal accuracy (AP-Acc) is defined as 
\begin{equation}
    AP\mhyphen Acc = \frac{1}{N}\times\sum_{s=1}^{N}\frac{n_{c}^s}{n^s}
\end{equation}
\paragraph{Overall accuracy}
Overall accuracy (O-Acc) is defined as
\begin{equation}
    O\mhyphen Acc = \frac{\sum_{s=1}^{N}{n_{c}^s}}{\sum_{i=1}^{N}{n^s}}
\end{equation}
\paragraph{Average personal weighted F1}
Average personal weighted F1 (APW-F1) is defined as 
\begin{equation}
    APW\mhyphen F1 = \frac{1}{N}\times\sum_{s=1}^{N}W\mhyphen F1^{s}
\end{equation}

==> src/feature_list.tex <==
\section{Detailed feature list}\label{appendix:feature}
This section will list all 42 mouse interaction features, 418 statistical features of students and 13 statistical features of questions which we used in our method in detail. We removed features whose values are always 0.

\subsection{Mouse movement features}\label{appendix:mouse}
Mouse movement features are generated from students' mouse trajectories when solving a problem in an online interactive question pool and assigned to interaction nodes. Features and their explanation are listed in Table~\ref{feature_list1}. 
\begin{table}[h!]
    \caption{Mouse movement features. GC denotes generalized clicks in Section~\ref{feature_extraction}. Think time is the thinking time of students before starting to answer the question. First attempt is the first action episode after think time. Features with * are categorical features encoded by one-hot encoding.}
\small
\vspace{-1em}
\begin{tabular}{@{}lll@{}}
    \toprule
        Feature Name & Explanation \\
    \hline\hline
        1stGCTimeLength & \begin{tabular}[c]{@{}l@{}}Time length between entering the question \\page and the 1st GC. \end{tabular} \\ 
    \hline
        1stGCTimePercent & \begin{tabular}[c]{@{}l@{}}Percentage of the duration of the 1st GC.\end{tabular} \\ 
        \hline
        1stGCEventStartIdx & \begin{tabular}[c]{@{}l@{}}Number of mouse events before the 1st GC. \end{tabular} \\ 
        \hline
        1stGCEventPercent & \begin{tabular}[c]{@{}l@{}}Percentage of mouse events before the 1st\\ GC among all 
        mouse events. \end{tabular} \\ 
        \hline
        1stGCEventEndIdx & \begin{tabular}[c]{@{}l@{}}Number of mouse events when the 1st GC \\ ends. \end{tabular} \\ 
    \hline
        GCCount & \begin{tabular}[c]{@{}l@{}}Total number of GCs. \end{tabular} \\ 
         \hline
        GCPerSecond & \begin{tabular}[c]{@{}l@{}} Average number of GCs per second.\end{tabular} \\
         \hline
        AvgTimeBtwGC & \begin{tabular}[c]{@{}l@{}}Average time between GC.\end{tabular} \\
 \hline        
        MedTimeBtwGC & \begin{tabular}[c]{@{}l@{}}Median value of time between GCs.\end{tabular} \\
        \hline
        StdTimeBtwGC & \begin{tabular}[c]{@{}l@{}}Standard deviation value of time between \\ GCs. \end{tabular}\\
         \hline
        OverallDistance & \begin{tabular}[c]{@{}l@{}}Total mouse trajectory length.\end{tabular} \\
        \hline
        InteractionHour* & \begin{tabular}[c]{@{}l@{}}Time point when students are solving the \\problem. For example, 1:00 pm.\end{tabular} \\
        \hline
        ThinkTimeLength & \begin{tabular}[c]{@{}l@{}}Time length of think time. \\For example, 3211ms.\end{tabular} \\
        \hline
        ThinkTimePercent & \begin{tabular}[c]{@{}l@{}}Percentage of think time in the total time.\\ For example, 15\%.\end{tabular} \\
        \hline
        ThinkTimeEventCount & \begin{tabular}[c]{@{}l@{}}Total number of mouse events during \\think time.\end{tabular} \\
        \hline
        ThinkTimeEventPercent & \begin{tabular}[c]{@{}l@{}}Percentage of mouse events during \\think time in all mouse events. \end{tabular} \\
        \hline
        1stAttemptEventCount & \begin{tabular}[c]{@{}l@{}}Number of mouse event during 1st \\ attempt to answer the    question.\end{tabular} \\
        \hline
        TotalTime & \begin{tabular}[c]{@{}l@{}}Total time used in answering a question.\end{tabular} \\
        \hline
        TotalEventCount & \begin{tabular}[c]{@{}l@{}}Number of mouse event in answering \\ a question.\end{tabular} \\
        \bottomrule
    \end{tabular}

    \label{feature_list1}
\end{table}
\subsection{Statistical features of students}\label{appendix:student}
Statistical features of students are generated from historical score records to reflect students' past performance on groups of questions and assigned to student nodes. Features and their explanation are listed in Table~\ref{feature_list2}.
\begin{table}[h!]
\caption{Statistical features of students.}
\centering
\small
\vspace{-1em}
% \begin{tabular}{p{2.2cm}p{2.8cm}p{2.4cm}}
\begin{tabular}{@{}lll@{}}

\toprule
Feature Name & Explanation & Example \\
\hline\hline

\# Total trials &  \begin{tabular}[c]{@{}l@{}}Number of a student's \\total trials.\end{tabular}& - \\\hline

\# 2nd trials & \begin{tabular}[c]{@{}l@{}}Number of a student's \\2nd trials.\end{tabular}& - \\\hline

\begin{tabular}[c]{@{}l@{}}\% Trials in \\{[}math dimension$\times$ \\grade$\times$difficulty{]} \end{tabular}& \begin{tabular}[c]{@{}l@{}}Percentage of trials on \\questions of certain \\math dimension, \\grade and difficulty \end{tabular}& \begin{tabular}[c]{@{}l@{}}\% Trials on spatial \\questions of grade\\ 5 and difficulty 5\end{tabular}\\\hline
\begin{tabular}[c]{@{}l@{}}Mean1stScore in \\{[}math dimension$\times$ \\grade$\times$difficulty{]} \end{tabular}& \begin{tabular}[c]{@{}l@{}}Mean score of 1st trials \\on questions of certain \\math  dimension,\\ grade and difficulty \end{tabular}& \begin{tabular}[c]{@{}l@{}}Mean1stScore on\\ numeric questions \\of grade 8 and\\ difficulty 3\end{tabular}\\
\bottomrule
\end{tabular}
\label{feature_list2}
\end{table}




\subsection{Statistical features of questions}\label{appendix:question}
Statistical features of questions are generated from historical score records and questions' predefined labels including \emph{difficulty}, \emph{math dimension} and \emph{grade}. These features are assign to question nodes. Features and their explanation are listed in Table \ref{feature_list3}.
\begin{table}[h!]
\caption{Statistical features of questions. Features with * are categorical features encoded by one-hot encoding.}
\centering
\small
\vspace{-1em}
% \begin{tabular}{p{1.8cm}p{3.2cm}p{2.2cm}}
\begin{tabular}{@{}lll@{}}
\toprule
Feature Name & Explanation & Example \\
\hline\hline
\begin{tabular}[c]{@{}l@{}}Math\\dimension* \end{tabular} & \begin{tabular}[c]{@{}l@{}} Question's related topic. \end{tabular} & Numeric \\\hline

Grade* & Grade of target students. & 12 \\\hline
Difficulty* & \begin{tabular}[c]{@{}l@{}}Question's difficulty level.\end{tabular}& 4 \\\hline

\# Total trials &  \begin{tabular}[c]{@{}l@{}} Number of trials on a \\ question.\end{tabular}& - \\\hline

\# 2nd trials & \begin{tabular}[c]{@{}l@{}}Number of 2nd trials on \\a question.\end{tabular}& - \\\hline

\begin{tabular}[c]{@{}l@{}}\% Trials getting\\ {[}score level{]} \end{tabular}& \begin{tabular}[c]{@{}l@{}}Percentage of trials in \\ each score level \end{tabular}& \% Trials getting 4\\
\bottomrule
\end{tabular}
\label{feature_list3}
\end{table}

==> src/intro.tex <==
\section{Introduction}
% Large-scale online learning environment is emerging in recent years for its advantages in fulfilling personal education need without spatial and temporal limits. Various form of such environment could be MOOC, intelligent tutoring systems and interactive online question pools. These learning platforms make it possible to collect and analysis massive students' information from not only traditional perspective including single student's historical records but distinctive aspects such as students' mouse movement and students' social network. To better utilize the collected data and help students, previous researchers have explored designing personal learning paths, identifying risky students, predicting the dropout rate and other applications. And the core problem of all these applications is to accurately predict the students' future performance on certain problems or courses.

% Traditional methods for students' performance estimation mostly use decision trees, support vector machines or linear regressions to learn the pattern of statistical features of both students and problems. However, these models highly related on the quality of handcrafted features and the input data is limited to 1D vectors. To further tackle the problem, recurrent neural networks (RNNs) have been introduced to this field and shows its ability to capture the temporal advance of students' knowledge. Recently, some researchers also pay attention on graph neural networks (GNNs) since its capability to learn more complex data structure i.e., graphs of undergraduate courses.

% All of the models mentioned above are mainly designed for well-designed curriculum such as undergraduate courses or predefined question order in MOOCs platforms and are not suitable for predicting students' performance in interactive online question pools. 

Large-scale online learning platforms are emerging in recent years for its advantages in fulfilling personal education need without spatial and temporal limits. Various forms of such platforms could be Massive Open Online Courses (MOOCs), intelligent tutoring systems and interactive online question pools. 
These learning platforms make it possible to collect and analyze massive students' information from not only traditional perspective including single student's historical records but distinctive aspects such as students' mouse movement and students' social network. 
To better utilize the collected data and help students, previous researchers have explored designing personal learning paths, identifying risky students, predicting the dropout rate and other applications. 
However, the core problem of all these applications is to accurately predict the students' future performance on certain questions or courses.


Traditional methods for students' performance estimation can be categorized into two classes
% following Hu's paper
~\cite{DBLP:conf/edm/HuR19}: static models and sequential models. Static models mainly include tree-based models\cite{Pardos12}, support vector machines\cite{ManriqueNMCN19} or linear regressions\cite{RenRJ16} to learn the pattern of statistical features of both students and questions. 
% and the input data is limited to 1D vectors.
% To further tackle the problem, sequential models have been introduced to this field and shows its ability to capture the temporal advance of students' knowledge. 
Sequential models focus on modeling the temporal evolution of student knowledge and these models include Bayesian Knowledge Tracing (BKT)~\cite{BKT0, BKT1} or Deep Knowledge Tracing (DKT)~\cite{DKT}, which are mainly based on recurrent neural networks (RNN).
% Recently, some researchers also pay attention on graph neural networks (GNNs) due to its capability to learn from more complex data structure and proposed AGCN\cite{DBLP:conf/edm/HuR19} to be applied on the homogeneous graphs of undergraduate courses with low-dimensional edge features.
The more recent research has also applied graph neural networks (GNNs) to student performance prediction on the homogeneous graphs of courses with low-dimensional edge features.

However, all the approaches mentioned above are designed for well-structured curriculum or questions with predefined order in MOOC platforms or undergraduate courses and are not suitable for predicting students' performance in online question pools, where the questions do not have a well-structured order or sequences.
Different from MOOCs, online question pools mainly aim to provide students with a collection of questions to practice their knowledge,
% serve as supplementary materials for practicing 
% so there are not any curriculums or question orders predefined by question designers.
where there are no pre-defined question orders by question designers. 
% Among all question pools, some of them use interactive questions, also called educational games, with multiple type of actions including drag-and-drops and clicks to raise the interest of K-12 students and these pools are often classified as interactive online question pools.
Among all question pools, some of them involve intense user interactions (e.g., mouse drag-and-drops, clicks) to increase the interest of students in working on the questions, which are often called \textit{interactive online question pools} or \textit{educational games}.
Interactive online question pools are getting more and more popular recently. For instance, interactive online question pools like Math Playground\footnote{\href{https://www.mathplayground.com/}{https://www.mathplayground.com/}} and Learnlex\footnote{\href{ https://mad.learnlex.com/login}{ https://mad.learnlex.com/login}} are gainning increasing attention from both teachers adn students.   
% , for example, LeetCode\footnote{\href{https://leetcode.com/}{\url{https://leetcode.com/}}} and  Math Playground\footnote{\href{https://www.mathplayground.com/}{https://www.mathplayground.com/}}, are getting popular recently but the research on students' performance prediction in them is still insufficient. 
However, research on accurate student performance prediction on interactive online question pools is still insufficient.
% Wei et al.~\cite{} has proposed a method to build a problem-solving network with students, questions and the interactions between them interactive online question pools and utilize the most similar questions to make prediction on other questions.
Wei et al.~\cite{} proposed novel features by incorporating student mouse movement interactions and similarities of questions to achieve better student performance prediction.
% a method to build a problem-solving network with students, questions and the interactions between them interactive online question pools and utilize the most similar questions to make prediction on other questions.
However, the major flaw of their method is that it can only achieve high accuracy when predicting the similar questions in a small dataset in which all questions can only have drag-and-drops.

To better handle the major challenge of making student performance prediction on interactive online question pools, we proposed a new set of interaction features extracted from mouse trajectories and designed a GNN-based approach, called R$^2$GCN, to compute on heterogeneous graphs with multi-dimensional edge features. Inspired by the interaction feature set of mouse trajectories proposed by Wei et al.~\cite{Wei2020lak}, we adapt the features related to \textit{'think-time'}, an important concept proposed by XXX, and change point detection. Furthermore, to address the problem that not all the interactive questions need drag-and-drop, we generalize the related features to suit clicks. Then we construct a problem-solving network which links students and questions by interactions.
% At last, our  R$^2$GCN is directly applied to the network to predict the students' performance on other unfinished questions.
Finally, we propose a graph neural networks based approach, called R$^2$GCN, to predict  students' performance on other unfinished questions. 
Specifically, the model first transforms all the interaction nodes to edges and further adapted RGCN~\cite{} to predict student performance on interactive online question pools by incorporating residual connection of graph convolution layers and wide \& deep\cite{wide&deep} model structure into our model architecture, enhancing the prediction performance.
% then applied some advanced techniques including residual connection of graph convolution layers and wide \& deep\cite{wide&deep} model structure to further improve the performance of prediction. 
% Finally, a
A real-world dataset, which is collected from a K-12 interactive online math question pool by our industry collaborator, is used to evaluate the prediction accuracy of our method in comparison with other the-state-of-the-art approaches. 

% Weighted F1 score and accuracy. We also compared our models' performance with the traditional models used in Wei's paper\cite{Wei2020lak} and other GNN models to show the effectiveness of our method.

The main contributions of this paper can be summarized as follows:

\begin{itemize}
	\item We propose a new approach based on graph neural network, called R$^2$GCN, for student performance prediction on interactive online question pools. It intrinsically works for the heterogeneous networks and can be used for training a personal model for different students on all the questions.
	
    \item We design a network to represent the relationship between students and questions by linking them with the interaction information in online interactive question pools. Furthermore, we utilize the technique, Edge2Node~\cite{}, to simplify the network for the application of GNNs. The method of network construction could also serve as a example for fields other than large scale online learning.
    
    \item We introduce new features to model student learning behaviors, which can extensively delineate student interactions including both drag-and-drop and clicks. 
    % We refine the previous interaction feature set and extend them to be used in various kinds of mouse events including both drag-and-drop and clicks.
    
    \item We conduct detailed evaluations of our approach on a real-world dataset. The result demonstrates their capability in achieving a better prediction accuracy than both traditional machine learning models and the graph convolutional neural network(GCN) model.
\end{itemize}
